The Milky Way's stellar streams and globular clusters do not align in a Vast Polar Structure

There is increasing evidence that a substantial fraction of Milky Way satellite galaxies align in a rotationally-supported plane of satellites, a rare configuration in cosmological simulations of galaxy formation. It has been suggested that other Milky Way substructures (namely young halo globular clusters and stellar/gaseous streams) similarly tend to align with this plane, accordingly dubbed the Vast Polar Structure (VPOS). Using systemic proper motions inferred from Gaia data, we find that globular cluster orbital poles are not clustered in the VPOS direction, though the population with the highest VPOS membership fraction is the young halo clusters (~30%). We additionally provide a current census of stellar streams, including new streams discovered using the Dark Energy Survey and Gaia datasets, and find that stellar stream normals are also not clustered in the direction of the VPOS normal. We also find that, based on orbit modeling, there is a likely association between NGC 3201 and the Gj\"{o}ll stellar stream and that, based on its orbital pole, NGC 4147 is likely not a Sagittarius globular cluster. That the Milky Way's accreted globular clusters and streams do not align in the same planar configuration as its satellites suggests that the plane of satellites is either a particularly stable orbital configuration or a population of recently accreted satellites. Neither of these explanations is particularly likely in light of other recent studies, leaving the plane of satellites problem as one of the more consequential open problems in galaxy formation and cosmology.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

